Knowledge Distillation from Multiple Foundation Models for End-to-End Speech Recognition

Although large foundation models pre-trained by self-supervised learning have achieved state-of-the-art performance in many tasks including automatic speech recognition (ASR), knowledge distillation (KD) is often required in practice to transfer the knowledge learned by large teacher models into much smaller student models with affordable computation and memory costs. This paper proposes a novel two-stage KD framework to distil the knowledge from multiple speech foundation models as teachers into a single student neural transducer model for ASR. In the first stage, the student model encoder is pre-trained using the embeddings extracted from multiple teacher models. In the second stage, the student encoder is fine-tuned with the audio-text pairs based on the ASR task. Experiments on the LibriSpeech 100-hour subset show that the proposed KD framework improves the performance of both streaming and non-streaming student models when using only one teacher. The performance of the student model can be further enhanced when multiple teachers are used jointly, achieving word error rate reductions (WERRs) of 17.5% and 10.6%. Our proposed framework can be combined with other existing KD methods to achieve further improvements. Further WERRs were obtained by incorporating extra unlabelled data during encoder pre-training, leading to a total relative WERR of 55.0% on the non-streaming student model.

==> figs/pretraining_data.tex <==
% to show only one bar in the legend
\pgfplotsset{compat=1.11,
    /pgfplots/ybar legend/.style={
    /pgfplots/legend image code/.code={%
       \draw[##1,/tikz/.cd,yshift=-0.25em]
        (0cm,0cm) rectangle (3pt,0.8em);},
   },
}

\begin{tikzpicture}
\begin{axis}[
    legend cell align={right},
    legend style={nodes={scale=0.7, transform shape}},
    width=0.33\textwidth,
    tick align=outside,
    tick pos=left,
    xlabel=Encoder pretraining data (hour),
    ylabel= Word error rates,
    xmin=0, xmax=2100,
    ymin=12, ymax=23,
    xtick={100,960, 2000},
    xticklabels={100,960, 2k},   % <---
    ytick={10,4,...,23}
            ]
\addplot[mark=*,black, mark size=1, densely dashdotted] 
plot coordinates {
    (100,21.2)
    (960,13.1)
    (2000,13.0)
};
\addlegendentry{HuBERT}

\addplot[color=black,mark=*, mark size=1, densely dashed]
    plot coordinates {
        (100,20.7)
        (960,12.9)
        (2000,12.8)
    };
\addlegendentry{WavLM}

\addplot[color=black,mark=x, mark size=1]
    plot coordinates {
        (100,19.5)
        (960,12.8)
        (2000,12.6)
    };
\addlegendentry{Hu+WavLM}
\end{axis}
%\caption{WER on test-other}
%\label{fig:werr_pretraining}
\end{tikzpicture}
% ---------------------------------------------------------------------------------------
\begin{tikzpicture}
\definecolor{darkgray176}{RGB}{176,176,176}
\begin{axis}[
legend cell align={left},
legend style={
    nodes={scale=0.7, transform shape},
  fill opacity=1.0,
  draw opacity=1.0,
  text opacity=1,
  at={(0.01,0.99)},
  anchor=north west,
  draw=none
},
width=0.33\textwidth,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Encoder pre-training data (hour)},
xmin=-0.23, xmax=2.63,
xtick style={color=black},
xtick={0.2,1.2,2.2},
xticklabels={100,960,2k},
y grid style={darkgray176},
ylabel={Averaged WERR (\%)},
ymin=0, ymax=40.46875,
ytick style={color=black},
]
\draw[draw=black,fill=white,postaction={pattern=north east lines}] (axis cs:-0.1,0) rectangle (axis cs:0.1,2.08333333333334);
\draw[draw=black,fill=white,postaction={pattern=north east lines}] (axis cs:0.9,0) rectangle (axis cs:1.1,35.0694444444444);
\draw[draw=black,fill=white,postaction={pattern=north east lines}] (axis cs:1.9,0) rectangle (axis cs:2.1,36.1111111111111);
\addlegendimage{ybar,ybar legend,draw=black,fill=white,postaction={pattern=north east lines}}
\addlegendentry{HuBERT}

\draw[draw=black,fill=white,postaction={pattern=north west lines}] (axis cs:1.1,0) rectangle (axis cs:1.3,36.1111111111111);
\draw[draw=black,fill=white,postaction={pattern=north west lines}] (axis cs:2.1,0) rectangle (axis cs:2.3,37.5);
\draw[draw=black,fill=white,postaction={pattern=north west lines}] (axis cs:0.1,0) rectangle (axis cs:0.3,4.86111111111112);
\addlegendimage{ybar,ybar legend,draw=black,fill=white,postaction={pattern=north west lines}}
\addlegendentry{WavLM}


\draw[draw=black,fill=white,postaction={pattern=crosshatch}] (axis cs:1.3,0) rectangle (axis cs:1.5,37.5);
\draw[draw=black,fill=white,postaction={pattern=crosshatch}] (axis cs:2.3,0) rectangle (axis cs:2.5,38.5416666666667);
\draw[draw=black,fill=white,postaction={pattern=crosshatch}] (axis cs:0.3,0) rectangle (axis cs:0.5,9.375);
\addlegendimage{ybar,ybar legend,draw=black,fill=white,postaction={pattern=crosshatch}}
\addlegendentry{Hu+WavLM}

\end{axis}
%\caption{Relative WERRs}
\label{fig:werr_pretraining}
\end{tikzpicture}
% ---------------------------------------------------------------------------------------
\begin{tikzpicture}
\begin{axis}[
    legend style={nodes={scale=0.7, transform shape}},
    width=0.33\textwidth,
    tick align=outside,
    tick pos=left,
    xlabel=Encoder pretraining data (hour),
    ylabel=averaged $L_1$ error,
    xmin=0, xmax=2100,
    ymin=0, ymax=0.5,
    xtick={100,960, 2000},
    xticklabels={100,960, 2k},   % <---
    ytick={0.1,0.05,...,0.4}
            ]
\addplot[mark=*,black, densely dashdotted] 
plot coordinates {
    (100,0.1667)
    (960,0.1490)
    (2000,0.1482)
};
\addlegendentry{HuBERT}

\addplot[color=black,mark=*, densely dashed]
    plot coordinates {
        (100,0.1511)
    (960,0.1332)
    (2000,0.13302)
    };
\addlegendentry{WavLM}

\addplot[color=black,mark=x]
    plot coordinates {
        (100,0.3095)
    (960,0.2988)
    (2000,0.2972)
    };
\addlegendentry{Hu+WavLM}
\end{axis}
%\caption{$L_1$ error}
\label{fig:l1_err_pretraining}
\end{tikzpicture}


==> text/6-discussion.tex <==
\section{Ablations}
\label{sec:ablations}

\subsection{Teacher Model Selection Strategy}

In this section, three teacher model selection strategies are compared. The first strategy is uniform sampling, i.e selecting each teacher with probability $p_n=\frac{1}{N}$. This strategy is also adopted in this work. However, this sampling method treats all teacher models equally, ignoring the performance difference between different teachers. To consider this, another sampling strategy can be applied:
\begin{align}
    % p_{n} = \frac{N-1}{N} \frac{\sum_{k=1,k\neq n }^{N} \text{WER}_{n}}{\sum_{k=1}^{N} \text{WER}_{n}},
    p_{n} = \frac{1}{N-1} \frac{\sum_{k=1,k\neq n }^{N} \text{WER}_{n}}{\sum_{k=1}^{N} \text{WER}_{n}},
\end{align}
where $\text{WER}_n$ is the $n$-th teacher model's WER on a pre-defined test set. Intuitively, teacher models with lower WERs will be more likely to be chosen than those with higher WERs. The third strategy assigns sampling probabilities by comparing the similarity between the student embedding and teacher embedding:
\begin{align}
    p_i =  \frac{\textsc{Sim}(\mathcal{E}^{\mathcal{T}_i}, \mathcal{E}^{\mathcal{S}})}{\sum_{n=1}^{N} \textsc{Sim}(\mathcal{E}^{\mathcal{T}_n}, \mathcal{E}^{\mathcal{S}})}
    \label{eqn:sim prob}
\end{align}
where $\textsc{Sim}$ is a normalised function that returns a higher value if two vectors are similar to each other. Intuitively, the teacher model whose embedding is more similar to the student embedding is more likely to be chosen.

\begin{table}[!ht]
    \centering
    \begin{tabular}{lccccc}
        \toprule
        \multirow{2}{*}{Teacher} & \multirow{2}{*}{\shortstack[c]{Sampling\\ method}}  & \multicolumn{2}{c}{dev}   & \multicolumn{2}{c}{test}  \\
        \cmidrule(lr){3-4}  \cmidrule(lr){5-6} &
        & \multicolumn{1}{c}{clean} & \multicolumn{1}{c}{other} & \multicolumn{1}{c}{clean} & \multicolumn{1}{c}{other} \\ 
        \midrule
        
        \multirow{3}{*}{W2v2+Hu} & uniform & 6.4 & 19.6 & 6.6 & 20.0 \\
        & WER & 6.4 & 19.6 & 6.6 & 20.0 \\
        & similarity & 6.6 & 20.0 & 6.8 & 20.4 \\
        \midrule
        \multirow{3}{*}{WL+Hu} & uniform  & 6.2 & 19.2 & 6.6 & 19.5 \\
        & WER & 6.2 & 19.3 & 6.6 & 19.5 \\
        & similarity & 6.4 & 19.9 & 6.8 & 20.2 \\
        
        \bottomrule
    \end{tabular}
    \caption{\%WERs for non-streaming student transducer models trained with different teacher model selection strategies under a multi-teacher setup.}
    \label{tab:teacher model selection 100h}
\end{table}


The results of three teacher model selection strategies described above are shown in \tbl{teacher model selection 100h}. The cosine similarity averaged over a number of acoustic frames was used in the similarity-based strategy. Two multi-teacher setups (W2v2+Hu, WL+Hu) were compared. In WER-based probability assignment strategies, the mean WER of dev-clean and dev-other was used. Experiments were carried out on the ``train-clean-100'' set. Sampling teacher models uniformly and assigning probabilities to teacher models based on their WERs yield almost the same performance. This could be explained by the small WER differences between different teacher models.  Choosing teacher labels by comparing the similarity between teacher embeddings and student embeddings yields the weakest performance. After a few epochs during training, it is observed that the selection of teacher labels converges slowly to one specific teacher. Then, the system degrades from multi-teacher to single-teacher, thus reducing the diversity of teacher labels and undermining KD training. 

In the future, we would like to further explore the WER-related sampling strategy. After vast amount of pre-training, the large foundation models all achieve very good performance after sufficient fine-tuning. The small WER differences between them make the WER-related sampling strategy very similar to uniform sampling. To simulate scenarios where teacher models have very different qualities, teacher models can be constructed by deliberately reducing the fine-tuning steps. This should help us investigate if a more sophisticated sampling strategy is better than uniform sampling.

% Different sampling mechanisms for choosing the target teacher model can be applied. The simplest sampling method would be assigning the same probability, i.e $p_{n}=1/N$, to all $N$ teachers. However, this sampling method treats all teacher models equally, ignoring the performance difference between different teachers. Therefore, an improved sampling method can be applied:
% \begin{align}
%     % p_{n} = \frac{N-1}{N} \frac{\sum_{k=1,k\neq n }^{N} \text{WER}_{n}}{\sum_{k=1}^{N} \text{WER}_{n}},
%     p_{n} = \frac{1}{N-1} \frac{\sum_{k=1,k\neq n }^{N} \text{WER}_{n}}{\sum_{k=1}^{N} \text{WER}_{n}},
% \end{align}
% where $\text{WER}_n$ is the $n$-th teacher model's WER on a pre-defined test set. Intuitively, teacher models with lower WERs will be more likely to be chosen than those with higher WERs.

% The selection of the teacher model can also be determined by the similarity between the teacher and student embeddings. If a student model's embedding is ``closer'' to one of the embeddings from the teacher pool, the student model would be able to adapt to that specific teacher model more easily. The probability of selecting the $i$-th teacher model can be expressed as:
% \begin{align}
%     p_i =  \frac{\textsc{Sim}(\mathcal{E}^{\mathcal{T}_i}, \mathcal{E}^{\mathcal{S}})}{\sum_{n=1}^{N} \textsc{Sim}(\mathcal{E}^{\mathcal{T}_n}, \mathcal{E}^{\mathcal{S}})}
%     \label{eqn:sim prob}
% \end{align}
% where $\textsc{Sim}$ is a normalised function that returns a higher value if two vectors are similar to each other. According to \eqndot{sim prob}, the teacher model whose embedding is more similar to the student embedding is more likely to be chosen. % as teacher targets.
